Only Large Weights (And Not Skip Connections) Can Prevent the Perils of Rank Collapse

Attention mechanisms lie at the heart of modern large language models (LLMs). Straightforward algorithms for forward and backward (gradient) computation take quadratic time, and a line of work initiated by [Alman and Song NeurIPS 2023] and [Alman and Song NeurIPS 2024] has shown that quadratic time is necessary unless the model weights are small, in which case almost linear time algorithms are possible. In this paper, we show that large weights are necessary to avoid a strong preclusion to representational strength we call layer collapse, which means that the entire network can be approximated well by a network with only a single layer. Thus, the quadratic running time of attention is unavoidable for expressive transformers. The notion of layer collapse that we introduce is a variant on the notion of rank collapse from the work of [Dong, Cordonnier, and Loukas ICML 2021]. They showed that in Self Attention Networks with small weights and with skip connections, rank collapse must occur. This is typically interpreted as justifying the necessity of skip connections in expressive networks. However, our result shows that even with skip connections, if the weights are small, then layer collapse still occurs. Thus, only large weights, and not skip connections, can prevent these representational weaknesses.

==> 03_tech.tex <==

\section{Technique Overview}


The tools developed in previous work \cite{dcl21} show that, when an input $X$ is passed through a single attention head, the resulting output has a small residual. In their setting \cite{dcl21}, where residual connections were not included, this observation was sufficient to prove their main results, since their lemma ensured that the residuals became smaller with each layer.

In this work, we aim to include residual connections in the transformer network. Lemma~\ref{lem:rank1_single_head} explains how to handle this starting from the second layer: now the input ($B$) to layer $\ell$ is the sum of the output of layer $\ell-1$ ($A$) and the input to layer $\ell-1$ ($X$). Our Lemma~\ref{lem:rank1_single_head} shows that, under this setup, the output of layer $\ell$ is still close to the output of layer $\ell-1$.

We also need to extend Lemma~\ref{lem:rank1_single_head} to handle the multi-head attention case. In this case, we are summing several different $A$s (one from each head), not just a single one. This generalization should be straightforward.

With this, we will argue that, in a full $\SAtt$ block with residuals, the output of each layer remains close to the output of the previous layer. Moreover, the difference between consecutive layers gets smaller as we go deeper. This is exactly what Lemma~\ref{lem:rank1_single_head} guarantees.

Our main theorem will then show the following: if we have a $\SAtt$ with residuals and $L$ layers, there exists another $\SAtt$ with residuals and only $L'$ layers, where $L' \ll L$ (possibly even $L' = 1$), that still gives a good approximation of the original network. More precisely, for any $L > L'$, and any $\SAtt$ with residuals and $L$ layers, there is a $\SAtt$ with residuals and $L'$ layers that approximates the original up to a small error.

